The Second Reactive Synthesis Competition (SYNTCOMP 2015)

We report on the design and results of the second reactive synthesis competition (SYNTCOMP 2015). We describe our extended benchmark library, with 6 completely new sets of benchmarks, and additional challenging instances for 4 of the benchmark sets that were already used in SYNTCOMP 2014. To enhance the analysis of experimental results, we introduce an extension of our benchmark format with meta-information, including a difficulty rating and a reference size for solutions. Tools are evaluated on a set of 250 benchmarks, selected to provide a good coverage of benchmarks from all classes and difficulties. We report on changes of the evaluation scheme and the experimental setup. Finally, we describe the entrants into SYNTCOMP 2015, as well as the results of our experimental evaluation. In our analysis, we emphasize progress over the tools that participated last year.

==> eptcsdata.tex <==
\providecommand{\firstpage}{27}
\providecommand{\publicationstatus}{\v{C}ern\'y, Kuncak, Madhusudan (Eds.): Fourth Workshop on\\ Synthesis (SYNT 2015)\\
EPTCS 202, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.202.4}{10.4204/EPTCS.202.4}}
\pdfoutput=1
\providecommand{\eptcs}{{\sl Electronic Proceedings in Theoretical Computer Science}}
\providecommand{\opa}{, Open Publishing Association}
\providecommand{\finishreference}[6]{#1 #2#3, pp. #4--#5, \doi{10.4204/EPTCS.#2.#6}}
\providecommand{\thisvolume}[2][\eptcs]{%
 \ifthenelse{\equal{#2}{3}}{\finishreference{#1}{202}{\opa}{98}{111}{7}}{%
 \ifthenelse{\equal{#2}{5}}{\finishreference{#1}{202}{\opa}{112}{119}{8}}{%
 this volume of #1\opa}}}

